Privacy-preserving Fine-tuning of Large Language Models through Flatness

The privacy concerns associated with the use of Large Language Models (LLMs) have grown recently with the development of LLMs such as ChatGPT. Differential Privacy (DP) techniques are explored in existing work to mitigate their privacy risks at the cost of generalization degradation. Our paper reveals that the flatness of DP-trained models' loss landscape plays an essential role in the trade-off between their privacy and generalization. We further propose a holistic framework to enforce appropriate weight flatness, which substantially improves model generalization with competitive privacy preservation. It innovates from three coarse-to-grained levels, including perturbation-aware min-max optimization on model weights within a layer, flatness-guided sparse prefix-tuning on weights across layers, and weight knowledge distillation between DP \& non-DP weights copies. Comprehensive experiments of both black-box and white-box scenarios are conducted to demonstrate the effectiveness of our proposal in enhancing generalization and maintaining DP characteristics. For instance, on text classification dataset QNLI, DP-Flat achieves similar performance with non-private full fine-tuning but with DP guarantee under privacy budget $\epsilon=3$, and even better performance given higher privacy budgets. Codes are provided in the supplement.

==> 1intro_old.tex <==

\section{Introduction}
Large Language Models(LLMs) have been widely used in the real world scenarios such as story generation~\cite{zhou2023recurrentgpt,yang2022re3}, AI agent~\cite{mialon2023augmented,da2023open} and Chatbots~\cite{luo2022critical}. ChatGPT and GPT4~\cite{OpenAI_GPT4_2023} have become part of life for human beings. However, previous works have already proven that LLMs will memorize the training data and leak the information from training data~\cite{carlini2021extracting,mireshghallah2022memorization}. Usually, the large amount of training data is collected from web and training data is likely to contain personal information such as e-mails~\cite{huang2022large}. Then leaking the training data may cause private information leakage. 

Such privacy issues for Large Language Models have extracted much attention~\cite{neel2023privacy}, and there are many methods that aims at protecting the data privacy. Among there methods, Differential Private (DP)~\cite{dwork2006calibrating,dwork2014algorithmic} is one of the most popular and standard paradigm to provide guarantee to data privacy. With well-chosen hyperparameters and Differentially Private Stochastic Gradient Descent (DP-SGD)~\cite{abadi2016deep} that provide DP guarantee to the training process, \citet{li2021large} has proven that LLMs can have a decent performance with tight DP guarantee and \citet{du2023dp} has proven that parameter efficient training methods such as prefix tuning~\cite{li2021prefix} can also fit well in the DP training framework. However, there still exists a performance gap between normal trained models and DP trained models for both full fine-tuning or parameter efficient training. Besides, \citet{li2021large} does not consider black-box optimization such as zeroth-order optimization~\cite{malladi2023fine}. Black-box optimization is very popular and important in LLMs because it not only reduces the training memory requirement~\cite{malladi2023fine}, but also can be applied to closed source models~\cite{chen2023instructzero}. 

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{images/flat_dp.pdf}
\caption{Weight loss landscape for DP trained LLMs on SST-2 and the results show that DP trained model has a sharper loss landscape. \hua{why this is not symmetric like other papers do?}}
\label{fig:flat}
\end{figure}


To further analyze the reason why there is a performance gap between normal training and DP training, we plot the loss landscape of Roberta~\cite{liu2019roberta} with normal training and DP training with DP-Adam on SST-2~\cite{socher2013recursive} in \cref{fig:flat}. We use the following formula to visualize the loss landscape with random Gaussian noise $\mathbf{d}$:
\begin{equation}
    f(\gamma) = \mathcal{L}(\mathcal{D}|\mathbf{w} + \gamma \mathbf{d}),
\end{equation}
where $\mathcal{D}$ and $\mathbf{w}$ are dataset and model weights respectively. The results clearly show that a DP-trained model has a sharper loss landscape. Besides, a flat loss landscape should help DP training since the noise added to the gradient will not influence the loss drop. Therefore, to improve the performance of a DP-trained LLMs, in this paper, we consider improving the flatness of the weight loss landscape from the following three aspects, in both black-box and white-box settings:

1) Weights within layer: First, we consider improving the flatness of the weights within each layer. The number of layers in LLMs does not influence
the effect of the proposed method. To improve the flatness of the weight loss landscape within layer, we utilize the method from \citet{wu2020adversarial} to explicitly flatten the weight loss landscape within each layer. 


2) Weights across layers: Then, we consider the influence of weights in different layers of LLMs on the flatness. To improve flatness through weights across layers, we consider sparse prefix-tuning for the white-box setting. Prefix tuning~\cite{li2021prefix} is a parameter-efficient training method that adds a prefix to each layer of LLMs. However, we find that injecting the prefix to certain layers instead of all layers can help to flatten the weight loss landscape. Therefore we propose the flatness indicator to guide choosing the proper layers to add prefixes. 


3) Weights with non-DP duplication: Non-DP duplication refers to the normally trained prefix, which has the same initialization as the DP-trained prefix but is trained without DP guarantees. In detail, we use a normal trained prefix to guide DP training with another regularization term. We train the normal prefix and DP prefix with the same initialization and target that DP trained prefix can have similar flatness on loss landscape with the normal trained prefix. %This is the reason why we call it cross duplication flatness. 

\begin{figure*}[h]
\centering
\includegraphics[width=0.7\textwidth]{images/threetype.png}
\caption{Our methods improve the flatness of weight loss landscape from three aspects: 1) Weights within layer, 2) Weights across layers and 3) Weights with non-DP duplication.}
\label{fig:show}
\end{figure*}

%In this paper, we adopt prefix tuning~\cite{li2021prefix} in white-box setting and prompt tuning~\cite{lester2021power} in black-box setting.  
In \cref{fig:show}, we show our overall framework and we summarize our contribution of \ours as follows:
\begin{itemize}
    \item We are the first to combine the flatness and DP training in the domain of LLMs and we adopt Adversarial Weight Perturbation (AWP)~\cite{wu2020adversarial} to transformers.
    \item We propose a flatness indicator to choose the proper layers where we can add prefixes to flatten weight loss landscape as well as a weight knowledge distillation method with non-DP prefixes.
    \item Comprehensive experiments in both black-box and white-box settings are conducted to show that our proposed methods can bridge the gap between normal-trained LLMs and DP-trained LLMs.
\end{itemize}







==> 3method_old.tex <==
\section{Methods}
\subsection{Background}
In this paper, we focus on the approximate-DP~\cite{dwork2014algorithmic} for providing the training process privacy:
\begin{definition}{$(\epsilon,\delta)$-DP}
A randomized algorithm $\mathcal{M}:\mathcal{X} \rightarrow \mathcal{Y}$ is $(\epsilon,\delta)$-differentially private if for
all adjacent datasets $X,X' \in \mathcal{X}$ and all $Y \in \mathcal{Y}, \mathbb{P}(\mathcal{M}(X) \in Y) \leq exp(\epsilon)\mathbb{P}(\mathcal{M}(X') \in Y) + \delta$.
\end{definition}
Specifically, when we talking about DP training in deep learning, $\mathcal{M}$ refers to any randomized optimization methods and $\mathcal{Y}$ refers to possible parameter space for models.

DP algorithm $\mathcal{M}$ aims at ensuring the outputs of two similar datasets are indistinguishable, so that attacker is not able to know the information about training dataset given model weights. $\epsilon, \delta$ are privacy budgets which measure how strong is the protection. Small values for $\epsilon$ and $\delta$ indicate a strong privacy protection.

To obtain a DP algorithm, the most widely used method is clipping per-sample gradient, sampling a random noise $z \sim N(0,\sigma^2 I)$ and adding $z$ to the accumulated clipped gradient. The variance parameter $\sigma^2$ is determined by several factors including total training steps, $\epsilon$ and $\delta$.


\subsection{White-box Setting}
In this section, we introduce our new training methods from three aspects: 1)within layer flatness, 2)cross layer flatness, 3)cross duplication flatness.

\textbf{Weights within layer} To improve flatness through weights within layer, we propose the flatness-aware training with warm-up. The method we used here aims at explicitly flattening loss landscape. The number of layers in LLMs does not influence the effect of the proposed method. Models with only one layer trained flatness-aware training can also get a flatter loss landscape, which is the reason we call it improving withing layer flatness. Similar to previous flatten method AWP~\cite{wu2020adversarial}, we consider the worst-case weight perturbation into LLMs. In detail, let $\mathbf{w}$ represents the trainable parameter of LLMs we used, $\mathcal{D}$ represents the training dataset and $\mathbf{v}$ is the weight perturbation. We aims at finding  $\textbf{v}$ so that:
\begin{equation}
    \textbf{v} = \arg \max_{\mathbf{v}} \mathcal{L}(\mathcal{D};\mathbf{w}+\mathbf{v})
\end{equation}
Unlike the original AWP with double-perturbation to both inputs and weights, here we only consider the perturbation to weights. And we can use one-step gradient ascent to obtain $\mathbf{v}$. Following by the original AWP, updated weights should come back to the center point again for the next start and the update follows:
\begin{equation}
    \mathbf{w} \leftarrow \mathbf{w}+\mathbf{v} - \eta \nabla_{\mathbf{w}+\mathbf{v}} \mathcal{L}(\mathcal{D};\mathbf{w}+\mathbf{v}) - \mathbf{v}.
\end{equation}
In this paper, we consider a warm-up mechanism to further utilize the our flatness-aware training.  Unlike adversarial training considered in \citet{wu2020adversarial}, there is no strong correlation between performance and flatness. We want a flat weight loss landscape because the noise required in the DP training will influence less in a flat loss landscape. Due to this feature, we only use flatness-aware training in the first a few round. After $T$ rounds, we can get a flat weight loss landscape of LLMs and we come back to the normal training to enjoy the benefits from flat weight loss landscape:
\begin{equation}
    \mathbf{w} \leftarrow \mathbf{w} - \eta \nabla_{\mathbf{w}} \mathcal{L}(\mathcal{D};\mathbf{w}).
\end{equation}
During the training process, the required noises are only added to the final gradient $\nabla_{\mathbf{w}+\mathbf{v}} \mathcal{L}(\mathcal{D};\mathbf{w}+\mathbf{v})$ or $\nabla_{\mathbf{w}} \mathcal{L}(\mathcal{D};\mathbf{w})$ while the noise will not be added to the process of computing $\mathbf{v}$.

\textbf{Weights across layers} In white-box setting, we will consider the prefix tuning~\cite{li2021prefix} with pre-trained LLMs. For original prefix tuning, we add the prefix to each layer of LLMs. However, we find that the flatness of weight loss landscape will increase significantly if we do not add prefix to some layers. Models with different layer numbers and architectures have different layers to add the prefix so that they can have a better flatness. The prefix added to different layers influences the following output and loss landscape, that is why we call it cross layer flatness. In this section, To approximate estimate which layer to add the prefix, we design a greedy step-wise elimination method. At first, we need to formally define the sharpness of a loss landscape similar to ~\citet{zhang2021flatness}:
\begin{definition}[sharpness]
$S:=\max(\mathcal{L}(\mathcal{D}|\mathbf{w}')-\mathcal{L}(\mathcal{D}|\mathbf{w}))$.
\end{definition}
Here $\mathbf{w}' \in \{ \mathbf{w} - \eta \nabla \mathcal{L}(\mathcal{D}|\mathbf{w})| \eta \in [0,1]\}$ and $\mathbf{w}'$ represents all the possible weights alone the direction of negative gradient. In practice, we choose 21 $\eta$ from $[0,1]$ uniformly and calculate the sharpness based on the maximum value of 21 losses.

Our proposed method will start from the full prefix tuning $\mathbf{w} = [\mathbf{w}_1,...,\mathbf{w}_n]$ where $\mathbf{w}_i$ represents the prefix added to $i$-th layer. We firstly compute the sharpness $S_0$ of full prefix tuning with a random initialization. Then we will remove one layer from full prefix tuning to get:
\begin{equation}
\label{eq:eli}
    \mathbf{w}_{-i} = [\mathbf{w}_1,..,\mathbf{w}_{i-1},\mathbf{w}_{i+1},..]
\end{equation}
Then we compute she sharpness of all $\mathbf{w}_{-i}$ to choose the $\mathbf{w}_{-i}$ so that $\mathbf{w}_{-i}$ has a lowest sharpness. We will continue this loop until the remained prefix meet our sparse requirement or the sharpness does not decrease any more. We compute all the sharpness with the same random initialization. After this greedy choosing procedure, we can train the sparse prefix only on chosen layers.

\textbf{Weights with non-DP duplication} In this section,  we want to use the information from model weights with a flat loss landscape. To explicitly guide the training with this information, we add a new term of loss function to force DP trained weights should be close to its duplicated weights which has a flatter loss landscape. In detail, we firstly train a LLM with normal training framework, and we will store the parameters of trainable weight $\textbf{w}_{nor}$ i.g prefix in this setting. $\textbf{w}_{nor}$ has the same the initialization and layers to insert the prefix, which is the reason why we call $\textbf{w}_{nor}$ as duplicated weights. Then we have the following new term of loss function:
\begin{equation}
    \mathcal{L}_g = \lVert \textbf{w} - \textbf{w}_{nor} \rVert_2.
\end{equation}
Therefore, the final loss function in the warm-up stage will be:
\begin{equation}
\label{eq:final}
    \mathcal{L}_f = \mathcal{L}(\mathcal{D}|\mathbf{w}+\mathbf{v})+ \lambda \mathcal{L}_g,
\end{equation}
where $\mathcal{L}$ can be any loss function in general such as cross-entropy loss for sentence classification tasks. Finally, we summarize our training pipeline for white-box setting in \cref{alg:white}.

\begin{algorithm}[h!]
   \caption{White-box DP training pipeline}
   \label{alg:white}
   \small
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} $\lambda$, $\eta$,warm-up epochs $E$, DP training total epochs $T_{dp}$, normal training epochs $T_{nor}$, elimination rounds $R$, random initialization prefix $\mathbf{w}= [\mathbf{w}_1,...,\mathbf{w}_n]$. 
   \FOR{$r=1$ {\bfseries to} $R$}
   \STATE $S_{min} = \infty$
   \STATE $P = 0$
   \FOR{$i=1$  {\bfseries to} $n$}
   \STATE Get  $\mathbf{w}_{-n}$ in \cref{eq:eli}
   \STATE Compute sharpness $S$ for $\mathbf{w}_{-n}$
   \IF{$S < S_{min}$}
   \STATE  $S_{min} = S$, $P=n$
   \ENDIF
   \ENDFOR
   \STATE  $\mathbf{w} \leftarrow  \mathbf{w}_{-P} $
   \ENDFOR
   \STATE $\mathbf{w}_{nor} = \mathbf{w}$
   \FOR{$t=1$ {\bfseries to} $T_{nor}$}
   \STATE $\mathbf{w}_{nor} \leftarrow \mathbf{w}_{nor}-\eta \nabla_{\mathbf{w}_{nor}} \mathcal{L}(\mathcal{D}|\mathbf{w}_{nor}) $
   \ENDFOR
   \FOR{$t=1$ {\bfseries to} $T$}
   \IF{$t <= E$}
   \STATE Compute $\mathbf{v}$
   \STATE  $\mathcal{L}_f = \mathcal{L}(\mathcal{D}|\mathbf{w}+\mathbf{v})+ \lambda  \lVert \textbf{w} - \textbf{w}_{nor} \rVert_2$
   \ELSE
   \STATE $\mathcal{L}_f = \mathcal{L}(\mathcal{D}|\mathbf{w})+ \lambda  \lVert \textbf{w} - \textbf{w}_{nor} \rVert_2$
   \ENDIF
   \STATE Update $\mathbf{w}$ with $\mathcal{L}_f$ and DP-Adam
   \ENDFOR
\end{algorithmic}
\end{algorithm}



\subsection{Black-box setting}
in this section, we will introduce our method to black-box settings including DP training method and optimization method.

\textbf{Zeroth-order Optimization} Zeroth-order~(ZO) optimizer estimates the gradient of neural networks using finite differences without any backpropagation. Recently, MeZO~\cite{malladi2023fine} investigates the application of Simultaneous Perturbation Stochastic Approximation (SPSA, \citet{119632}), a classic ZO gradient estimation technique, to fine-tune LLMs. Given a model parameterized by $\mathbf\theta \in \mathbb R^{d}$ and a defined loss function $\mathcal L$, MeZO estimates the gradient over a minibatch $\mathcal B$ as follows:
\begin{equation}
\label{eq:mezo}
\begin{aligned}
    \hat\nabla\mathcal L(\mathbf \theta;\mathcal B) &=  \frac{\mathcal L(\mathbf \theta + \varepsilon\mathbf z;\mathcal B) - \mathcal L(\mathbf \theta - \varepsilon\mathbf z;\mathcal B)}{2\varepsilon}\mathbf z \\
    &\approx \mathbf z\mathbf z^\top \nabla\mathcal L(\mathbf \theta;\mathcal B) 
\end{aligned}
\end{equation}
where $\mathbf z\in \mathbb R^{d}$ with $\mathbf z \sim \mathcal N(0, \mathtt I_d)$ and $\varepsilon$ is the perturbation scale.  After obtaining the estimated gradient $\hat\nabla\mathcal L(\mathbf \theta;\mathcal B)$, MeZO proceeds to update the model parameters using the standard SGD rule: $\mathbf \theta_{t+1} = \mathbf \theta_t - \eta\hat\nabla\mathcal L(\mathbf \theta;\mathcal B_t)$, where $\eta$ is the learning rate.


\textbf{DPZero} We could directly add noise to the gradient obtained by the MeZO to ensure a DP guarantee, which means DP noise $\mathbf{g}$ is sampled from $\mathcal N(0, \sigma^2 \mathtt I_d)$ and added to $\hat\nabla\mathcal L(\mathbf \theta;\mathcal B)$ in \cref{eq:mezo}. However, this method poses dimension-dependent complexity, which makes the performance of combining DP training and zeroth order optimization suffers in high dimension~\cite{zhang2023dpzero}. To tackle the problem, DPZero~\cite{zhang2023dpzero} is the proposed. We directly use DPZero in our paper. Specifically, let $\mathbf{g}$ represent the noise from Gaussian distribution $N(0,\sigma^2)$, the gradient will be:
\begin{equation}
    \hat\nabla\mathcal L(\mathbf \theta;\mathcal B) &=  (\frac{\mathcal L(\mathbf \theta + \varepsilon\mathbf z;\mathcal B) - \mathcal L(\mathbf \theta - \varepsilon\mathbf z;\mathcal B)}{2\varepsilon}+\mathbf{g})\mathbf z
\end{equation}
Compared with directly combining DP mechanism with zeroth order optimization, DPZero only add noise to one direction so that it influences the update less. \citet{zhang2023dpzero} also proves with the same variance $\sigma^2$, DPZero achieve the same DP guarantee compared with DP-SGD.

\textbf{Weights with non-DP duplication} To adopt the method that improves flatness across layers, we need to add prefix to each layer, which is not practical to the black-box setting. Besides, we need to estimate two gradients if we want to improves through weights within layer. Therefore, in the black-box setting, we only consider using improving through non-DP duplication. Compared with white-box setting, $\textbf{w}_{nor}$ is also trained with black-box setting, and we treat \cref{eq:final} as the loss function in \cref{eq:mezo} to adopt our methods.

